Cascaded Beam Search: Plug-and-Play Terminology-Forcing For Neural Machine Translation

This paper presents a plug-and-play approach for translation with terminology constraints. Terminology constraints are an important aspect of many modern translation pipelines. In both specialized domains and newly emerging domains (such as the COVID-19 pandemic), accurate translation of technical terms is crucial. Recent approaches often train models to copy terminologies from the input into the output sentence by feeding the target terminology along with the input. But this requires expensive training whenever the underlying language model is changed or the system should specialize to a new domain. We propose Cascade Beam Search, a plug-and-play terminology-forcing approach that requires no training. Cascade Beam Search has two parts: 1) logit manipulation to increase the probability of target terminologies and 2) a cascading beam setup based on grid beam search, where beams are grouped by the number of terminologies they contain. We evaluate the performance of our approach by competing against the top submissions of the WMT21 terminology translation task. Our plug-and-play approach performs on par with the winning submissions without using a domain-specific language model and with no additional training.

==> abstract_submission.tex <==
This paper presents a plug-and-play approach for translation with terminology constraints. Terminology constraints are an important aspect of many modern translation pipelines. In both specialized domains and newly emerging domains (such as the COVID-19 pandemic), accurate translation of technical terms is crucial. Recent approaches often train models to copy terminologies from the input into the output sentence by feeding the target terminology along with the input. But this requires expensive training whenever the underlying language model is changed or the system should specialize to a new domain. We propose Cascade Beam Search, a plug-and-play terminology-forcing approach that requires no training. Cascade Beam Search has two parts: 1) logit manipulation to increase the probability of target terminologies and 2) a cascading beam setup based on grid beam search, where beams are grouped by the number of terminologies they contain. We evaluate the performance of our approach by competing against the top submissions of the WMT21 terminology translation task. Our plug-and-play approach performs on par with the winning submissions without using a domain-specific language model and with no additional training.

==> beamanalysis.tex <==
In Figure~\ref{fig:numbeam} we analyze the effect of the number of beams per cascade level on the performance of the proposed Cascade BeamSearch approach. In general we can observe an upwards trend for more beams, however even for as small as two or three beams the performance is acceptable.

\clearpage

==> comparison.tex <==

\section{Logit Manipulation} \label{sec:logman}


In Figure~\ref{fig:scaling_law} we can see the deteriorating effect that default logit manipulation has on the translation quality. We devise two strategies to push tokens. With strategy A only the longest possible token that starts/continues is pushed. With strategy B all possible tokens that start/continue a terminology are pushed. An example: For the word "COVID" the M2M100 tokenizer has the possibilities to produce C, CO but it can\'t produce any of COV, COVI or COVID. With strategy A we would push the token CO, with strategy B both C and CO. In Subfigure~\ref{fig:atermltok} we can see the results for Strategy A, in Subfigure~\ref{fig:atermatok} the results for Strategy B.

For both strategies we can observe that the EMA increases with stronger forcing and reaches values around 0.99 for a forcing weight of 1.0. Meanwhile, the BLEU score starts decreasing more and more with a stronger forcing. Indeed, during our experiments we observe that for examples with many terminologies too many beams are processing terminologies, while sensible sentence starts that do not contain any terminology are not developed during the beamsearch.

\newpage


==> related_work.tex <==


With the rise of Neural Machine Translation (NMT), trained on huge parallel corpora of multilingual text, the need for accurate terminology translation has also become more apparent. While translation engines are trained to be generalists, the domains where accurate translation of terminology is critical are plentiful. In a recent WMT21 shared task on terminology translation, almost all competitors use an approach where the target terminology is added to the source sentence, either behind the source terminology or at the end of the source sentence \citep{target_lemma, promt, ballier-etal-2021-spectrans, lingua_custodia, jon-etal-2021-cuni-systems, termmind, tilde, pham-etal-2021-systran, bak-etal-2021-kakao}.


Huge language generation models such as GPT-3 \citet{gpt3, PaLM} have revolutionized text generation in recent years. However, with these models becoming more and more powerful the interest in controlling them also becomes more interesting. While prompting has been one actively researched direction recently, another set of research explored the ability to modify the language models' logit outputs and guide the appearance of words through a modification of the decoding algorithm. \citet{pascual-etal-2021-plug-play} propose a setup where words can either be encouraged to appear (soft) or be required to appear (hard). In the latter approach, the logit manipulation is slowly made stronger the longer a terminology does not appear.

% \subsection{Grid Beamsearch}

% \citet{hokamp-liu-2017-lexically} introduce Grid BeamSearch, an approach very similar to the proposed Cascaded BeamSearch. Banks of beams containing more and more constraints are separately kept and can guarantee the appearance of all terminologies at the highest level. Each beam can either be in an open state, where outputs from the model can be generated or new terminologies can be started, or in a closed state, where active terminologies must be continued.


==> tables/bakcup.tex <==
%% Scaling_Law
% M5 - Train
% linear-descC100-L4-E1_valid__mae__epoch9999__test
% 0.880 (1.78) & 0.947 (1.96)  & 1.400 (1.67)
% linear-descC50-L4-E1_valid__mae__epoch9999__test
% 0.881 (1.78) & 0.948 (1.97)  & 1.403 (1.68)
% linear-descC10-L4-E1_valid__mae__epoch9999__test
% 0.881 (1.79) & 0.947 (1.97)  & 1.402 (1.68)
% linear-descC5-L4-E1_valid__mae__epoch9999__test
% 0.881 (1.78) & 0.947 (1.97)  & 1.403 (1.68)
% linear-descC2-L4-E1_valid__mae__epoch9999__test
% 0.882 (1.79) & 0.948 (1.98)  & 1.409 (1.69)

% UOC - 100K - 
% linear-descCsame100-L4-E1__mae__epoch9999__test
% 0.880 (2.87) & 0.920 (5.69)  & 1.233 (5.44)
% linear-descCsame50-L4-E1__mae__epoch9999__test
% 0.881 (2.88) & 0.921 (5.65)  & 1.235 (5.40)
% linear-descCsame10-L4-E1__mae__epoch9999__test
% 0.883 (2.87) & 0.927 (5.63)  & 1.233 (5.39)
% linear-descCsame5-L4-E1__mae__epoch9999__test
% 0.885 (2.87) & 0.927 (5.64)  & 1.241 (5.39)
% linear-descCsame2-L4-E1__mae__epoch9999__test
% 0.888 (2.87) & 0.935 (5.65)  & 1.240 (5.40)


%% Large
% M5 - Train
% lstm512-4
% 0.894 (1.82) & 0.968 (2.05)  & 1.447 (1.75)
% lstm5120_4-large__all__mae
% 0.903 (1.83) & 0.989 (2.08)  & 1.460 (1.78)
% lstm512_400-large__all__mae
% 1.073 (1.77) & 1.110 (2.22)  & 1.555 (1.93)

% UOC - 100K
% lstm512-4
% 0.946 (2.84) & 0.992 (5.84)  & 1.267 (5.58)
% lstm5120_4-large__all__mae
% 1.088 (3.16) & 1.516 (8.45)  & 1.878 (8.05)
% lstm512_400-large__all__mae
% 1.118 (2.98) & 1.201 (6.44)  & 1.466 (6.15)

==> tables/tab_ablation.tex <==
\begin{table*}[ht]
\centering
\caption{Ablation studies on Forchestra: Effectiveness of initialization.}
\label{tab:ablation}
{\normalsize
\begin{tabular}{l|ccc|ccc}
\toprule
\multirow{2}{*}{Model} & \multicolumn{3}{c|}{\texttt{E-Commerce}} & \multicolumn{3}{c}{\texttt{M5}}  \\
                      & MASE & MAE & RMSE         & MASE & MAE & RMSE       \\
\midrule
\bf Forchestra &  \bf 0.880 (2.87) & \bf 0.920 (5.69)  & \bf 1.233 (5.44) & \bf 0.880 (1.78) & \bf 0.947 (1.96)  & \bf 1.400 (1.67) \\
\midrule
Freezing rep. module of NC & 0.882 (2.88) & 0.922 (5.72)  & 1.238 (5.46) & 0.882 (1.78) & 0.949 (1.97)  & 1.405 (1.68) \\
\makecell[l]{Freezing rep. module of NC \\ + w/o Pre-training BPs \\ }       & 0.882 (2.88) & 0.927 (5.72)  & 1.244 (5.47) & 0.886 (1.78) & 0.957 (2.00)  & 1.411 (1.71) \\
\midrule
w/o Pre-training BPs \& NC  & 0.882 (2.89) & 0.925 (5.80)  & 1.246 (5.54) & 0.889 (1.79) & 0.960 (2.01)  & 1.426 (1.71) \\
w/o Pre-training NC         & 0.883 (2.88) & 0.924 (5.71)  & 1.238 (5.46) & 0.886 (1.78) & 0.957 (1.99)  & 1.415 (1.70) \\
w/o Pre-training BPs        & 0.884 (2.90) & 0.930 (5.82)  & 1.256 (5.56) & 0.895 (1.79) & 0.973 (2.03)  & 1.435 (1.74) \\
% \midrule
% w/ Random Grouping & 0.881 (2.87) & 0.921 (5.65)  & 1.232 (5.40) & 0.882 (1.79) & 0.948 (1.97)  & 1.402 (1.67) \\
% w/ Category Grouping & 0.885 (2.86) & 0.929 (5.66)  & 1.236 (5.41) & 0.882 (1.79) & 0.949 (1.97)  & 1.406 (1.68) \\
\bottomrule
\end{tabular}
}
\end{table*}


==> tables/tab_ablation_stale.tex <==
\begin{table*}[ht]
\centering
\caption{Ablation Studies. MAYBE WE CAN MAKE BAR PLOT FOR THIS!}
\label{tab:ablation}
{\small
\begin{tabular}{l|ccc|ccc}
\toprule
\multirow{2}{*}{Model} & \multicolumn{3}{c|}{\texttt{E-Commerce}} & \multicolumn{3}{c}{\texttt{M5}}  \\
                       & MASE & MAE & RMSE         & MASE & MAE & RMSE       \\
\midrule
\bf Forchestra ($K=10$) &  \bf 0.882 (2.88) & 0.927 (5.68)  & 1.242 (5.43) & \bf 0.881 (1.79) & \bf 0.947 (1.97)  & \bf 1.402 (1.68) \\
\midrule
% w/o BPs \& NC Fine-tuning & 0.891 (2.90) & 0.943 (5.75)  & 1.256 (5.49) & 0.882 (1.79) & 0.949 (1.99)  & 1.410 (1.69) \\
% w/o BPs Fine-tuning & 0.886 (2.89) & 0.931 (5.72)  & 1.246 (5.47) & 0.889 (1.78) & 0.962 (2.00)  & 1.420 (1.71) \\
w/o NC Fine-tuning & \bf 0.882 (2.89) & \bf 0.921 (5.72)  & \bf 1.237 (5.46) & 0.882 (1.79) & 0.949 (1.99)  & 1.410 (1.69) \\
% \midrule
w/o BPs \& NC Initialization      & 0.889 (2.90) & 0.938 (5.80)  & 1.259 (5.54) & 0.887 (1.79) & 0.959 (2.02)  & 1.420 (1.73) \\
w/o BPs Initialization      & 0.893 (2.90) & 0.957 (5.95)  & 1.277 (5.68) & 0.888 (1.77) & 0.956 (1.97)  & 1.402 (1.68) \\
w/o NC Initialization      & 0.896 (2.89) & 0.955 (5.80)  & 1.262 (5.54) & 0.884 (1.78) & 0.953 (1.97)  & 1.403 (1.68) \\
% \midrule
% w/ Random Grouping & 0.881 (2.87) & 0.921 (5.65)  & 1.232 (5.40) & 0.882 (1.79) & 0.948 (1.97)  & 1.402 (1.67) \\
% w/ Category Grouping & 0.885 (2.86) & 0.929 (5.66)  & 1.236 (5.41) & 0.882 (1.79) & 0.949 (1.97)  & 1.406 (1.68) \\
\bottomrule
\end{tabular}
}
\end{table*}

==> tables/tab_ens.tex <==
\begin{table*}[ht]
\centering
\caption{Comparison of forecast accuracy between Forchestra and ensemble approaches. The highest scores among ensemble methods are underlined.}
\label{tab:ens}
{\normalsize
\begin{tabular}{ll|ccc|ccc}
\toprule
\multirow{2}{*}{Approach}         & \multirow{2}{*}{Model} & \multicolumn{3}{c|}{\texttt{E-Commerce}} & \multicolumn{3}{c}{\texttt{M5}}  \\
                          &                        & MASE & MAE & RMSE         & MASE & MAE & RMSE       \\
\midrule
\bf Orchestra                  & \bf Forchestra &  \bf 0.880 (2.87) & \bf 0.920 (5.69)  & \bf 1.233 (5.44) & \bf 0.880 (1.78) & \bf 0.947 (1.96)  & \bf 1.400 (1.67) \\
\midrule
\multirow{3}{*}{\makecell[l]{Divide-and- \\ Conquer}} & Forch.+DnC (Fine-tuned) &  0.880 (2.88) & 0.920 (5.71)  & 1.236 (5.46) & 0.881 (1.78) & 0.947 (1.97)  & 1.403 (1.67) \\
& Forch.+DnC (Frozen) & 0.887 (2.88) & 0.938 (5.75)  & 1.245 (5.50) & 0.886 (1.78) & 0.955 (1.99)  & 1.409 (1.70) \\
 &  DnC & 0.899 (2.93) & 0.953 (5.94)  & 1.274 (5.67) & 0.889 (1.78) & 0.962 (2.00)  & 1.420 (1.71) \\
\midrule

\multirow{9}{*}{\makecell[l]{Ensemble \\ (global)}} 
                          & Average    & 0.905 (2.92) & 0.980 (5.96)  & 1.313 (5.69) & 0.890 (1.79) & 0.962 (2.03)  & 1.432 (1.73)) \\
                          & Top-50 & 0.922 (2.95) & 0.995 (5.98)  & 1.333 (5.70) & \underline{0.886 (1.79)} & \underline{0.955 (1.99)}  & 1.415 (1.70) \\
                          & Top-10 & 0.906 (2.92) & 0.982 (6.00)  & 1.311 (5.73) & 0.889 (1.79) & 0.959 (1.98)  & \underline{1.413 (1.68)} \\
                          & Top-5 & 0.905 (2.92) & 0.974 (5.92)  & 1.303 (5.65) &  0.890 (1.80) & 0.961 (2.00)  & 1.417 (1.70) \\
                          & Top-2 & \underline{0.904 (2.92)} & \underline{0.964 (5.82)}  & \underline{1.293 (5.56)} & 0.893 (1.79) & 0.965 (1.99)  & 1.414 (1.70) \\
                          & Top-1 & 0.908 (2.92) & 1.004 (6.08)  & 1.334 (5.81) & 0.894 (1.79) & 0.971 (2.04)  & 1.429 (1.75) \\
                          & W-inv & 0.914 (2.93) & 0.992 (5.98)  & 1.327 (5.71) & 0.890 (1.79) & 0.962 (2.03)  & 1.431 (1.73) \\
                          & W-sqr & 0.920 (2.94) & 1.000 (5.99)  & 1.337 (5.72) & 0.889 (1.79) & 0.961 (2.02)  & 1.430 (1.72) \\
                          & W-exp & 0.914 (2.93) & 0.991 (5.98)  & 1.327 (5.71) & 0.890 (1.79) & 0.962 (2.03)  & 1.431 (1.73) \\
\midrule
\multirow{8}{*}{\makecell[l]{Ensemble \\ (instance-wise)}} 
                          & Top-50 & 0.916 (2.93) & 0.977 (5.89)  & 1.318 (5.62) & 0.894 (1.79) & 0.964 (1.99)  & 1.421 (1.70) \\
                          & Top-10 & 0.916 (2.93) & 0.973 (5.82)  & 1.302 (5.55) & 0.902 (1.78) & 0.980 (2.02)  & 1.436 (1.73) \\
                          & Top-5 & 0.924 (2.95) & 0.986 (5.87)  & 1.314 (5.61) & 0.910 (1.79) & 0.993 (2.04)  & 1.449 (1.75) \\
                          & Top-2 & 0.944 (2.98) & 1.014 (5.95)  & 1.344 (5.68) & 0.929 (1.81) & 1.019 (2.09)  & 1.480 (1.79) \\
                          & Top-1 & 0.969 (3.05) & 1.057 (6.16)  & 1.390 (5.88) & 0.949 (1.84) & 1.049 (2.16)  & 1.521 (1.86) \\
                          & W-inv & 0.937 (3.47) & 1.120 (22.25)  & 1.449 (21.32) & 0.889 (1.79) & 0.959 (2.01)  & 1.426 (1.71) \\
                          & W-sqr & 0.939 (3.48) & 1.118 (22.24)  & 1.449 (21.31) & 0.889 (1.79) & 0.958 (2.01)  & 1.424 (1.71) \\
                          & W-exp & 0.932 (3.47) & 1.116 (22.25)  & 1.444 (21.32) & 0.889 (1.79) & 0.959 (2.01)  & 1.427 (1.72) \\
\bottomrule
\end{tabular}
}
\end{table*}


==> tables/tab_ens_stale.tex <==
\begin{table*}[ht]
\centering
\caption{Comparison of forecast accuracy between classical ensemble approaches and Forchestra ($K=10$) on the original dataset by using base predictors trained.}
\label{tab:ens}
{\small
\begin{tabular}{cl|ccc|ccc}
\toprule
\multirow{2}{*}{}         & \multirow{2}{*}{Model} & \multicolumn{3}{c|}{\texttt{E-Commerce}} & \multicolumn{3}{c}{\texttt{M5}}  \\
                          &                        & MASE & MAE & RMSE         & MASE & MAE & RMSE       \\
\midrule
\bf Orchestra                 & \bf Forchestra &  \bf 0.882 (2.88) & \bf 0.927 (5.68)  & \bf 1.242 (5.43) & \bf 0.881 (1.79) & \bf 0.947 (1.97)  & \bf 1.402 (1.68) \\
\midrule
Divide-and-Conquer & Segmentation & 0.899 (2.93) & 0.953 (5.94)  & 1.274 (5.67) & 0.889 (1.78) & 0.962 (2.00)  & 1.420 (1.71) \\
\midrule
\multirow{7}{*}{\makecell{Ensemble \\ (global)}} & Average    & 0.903 (2.92) & 0.983 (6.00)  & 1.314 (5.73) & 0.883 (1.78) & 0.952 (1.99)  & 1.410 (1.70) \\
                          & Top-1 & 0.891 (2.90) & 0.949 (5.86)  & 1.272 (5.59) & 0.885 (1.79) & 0.954 (2.00)  & 1.416 (1.70) \\
                          & Top-5 & 0.891 (2.90) & 0.949 (5.86)  & 1.272 (5.59) & 0.885 (1.79) & 0.954 (2.00)  & 1.416 (1.70) \\
                          & Top-10 & 0.891 (2.90) & 0.949 (5.86)  & 1.272 (5.59) & 0.885 (1.79) & 0.954 (2.00)  & 1.416 (1.70) \\
                          & Top-50 & 0.891 (2.90) & 0.949 (5.86)  & 1.272 (5.59) & 0.885 (1.79) & 0.954 (2.00)  & 1.416 (1.70) \\
                          & w-inv & 0.901 (2.92) & 0.978 (5.98)  & 1.309 (5.71) & 0.883 (1.78) & 0.952 (1.99)  & 1.410 (1.70) \\
                          & w-sqr & 0.900 (2.92) & 0.974 (5.96)  & 1.304 (5.69) & 0.883 (1.78) & 0.952 (1.99)  & 1.410 (1.70) \\
                          & w-exp & 0.901 (2.92) & 0.977 (5.98)  & 1.307 (5.71) & 0.883 (1.78) & 0.952 (1.99)  & 1.410 (1.70) \\
\midrule
\multirow{7}{*}{\makecell{Ensemble \\ (instance-wise)}} & Top-1 & 0.907 (2.93) & 0.963 (5.87)  & 1.291 (5.61) & 0.899 (1.78) & 0.977 (2.02)  & 1.435 (1.73) \\
                          & Top-5 & 0.891 (2.90) & 0.949 (5.86)  & 1.272 (5.59) & 0.885 (1.79) & 0.954 (2.00)  & 1.416 (1.70) \\
                          & Top-10 & 0.891 (2.90) & 0.949 (5.86)  & 1.272 (5.59) & 0.885 (1.79) & 0.954 (2.00)  & 1.416 (1.70) \\
                          & Top-50 & 0.891 (2.90) & 0.949 (5.86)  & 1.272 (5.59) & 0.885 (1.79) & 0.954 (2.00)  & 1.416 (1.70) \\
                          & w-inv & 0.900 (2.92) & 0.971 (6.12)  & 1.300 (5.84) & 0.884 (1.78) & 0.952 (1.99)  & 1.411 (1.70) \\
                          & w-sqr & 0.898 (2.91) & 0.961 (6.08)  & 1.289 (5.81) & 0.884 (1.78) & 0.953 (2.00)  & 1.411 (1.70) \\
                          & w-exp & 0.900 (2.91) & 0.974 (6.11)  & 1.304 (5.83) & 0.884 (1.78) & 0.952 (1.99)  & 1.411 (1.70) \\
\bottomrule
\end{tabular}
}
\end{table*}


==> tables/tab_ranking.tex <==
\begin{table*}[ht]
\caption{Rank-biased overlap (RBO) score between Forchestra and ensemble approaches.
}
\label{tab:ranking}
{\normalsize
\begin{tabular}{l|ccc|ccc}
\toprule
\multirow{2}{*}{Model} & \multicolumn{3}{c|}{\texttt{E-Commerce}} & \multicolumn{3}{c}{\texttt{M5}}  \\
                       & RBO@5 & RBO@10 & RBO@50 & RBO@5 & RBO@10 & RBO@50       \\
\midrule
Forchestra & 0.0093 & 0.0294 & 0.0931 & 0.0183 & 0.0390 & 0.1058 \\
\midrule
\makecell[l]{Ranked by val. score (global)} & 0.0148 & 0.0363 & 0.1013 & 0.0112 & 0.0352 & 0.1121 \\
\midrule
\makecell[l]{Ranked by val. score (instance-wise)} & 0.1770 & 0.3085 & 0.5317 &  0.0511 & 0.1030 & 0.2249 \\
% \midrule
% \makecell[l]{For comparison: \\ Ranked in a random order} & 0.0114 & 0.0303 & 0.097 & 0.0114 & 0.0303 & 0.097 \\
\bottomrule
\end{tabular}
}
\end{table*}


==> tables/tab_transfer.tex <==
\begin{table*}[t!]
\centering
\caption{Forecast accuracy on downstream dataset (i.e., unseen products). Models performing zero-shot inference are trained on the original dataset.}
\label{tab:comp_test}
{\normalsize
\hspace{-3em}
\begin{tabular}{r@{\,}ll|ccc|ccc}
\cmidrule[1.0pt]{2-9}
\multirow{2}{*}{}         & & \multirow{2}{*}{Model} & \multicolumn{3}{c|}{\texttt{E-Commerce} (Unseen Products)} & \multicolumn{3}{c}{\texttt{M5} (Unseen Products)}  \\
                          & &                        & MASE & MAE & RMSE         & MASE & MAE & RMSE       \\
\cmidrule{2-9}
\ldelim\{{12}{*}[\color{black} {\rotatebox[origin=c]{90}{trained on downstream dataset}}\hspace{.45em}]\hspace{.3em}
 & \multirow{3}{*}{Local} & ARIMA                  & 1.045 (1.84) & 0.987 (3.83)  & 1.202 (4.01) & 1.108 (1.67) & 1.163 (2.36)  & 1.482 (2.17) \\
                          & & Prophet                & 1.112 (1.97) & 1.126 (4.21)  & 1.356 (4.34) & 1.125 (1.66) & 1.172 (2.08)  & 1.501 (1.86) \\
                          & & SMA         & 1.145 (2.15) & 1.179 (4.60)  & 1.396 (4.69) & 1.180 (1.92) & 1.413 (2.75)  & 1.843 (2.48) \\
\cmidrule{2-9}
& \multirow{6}{*}{Global} & DeepAR             & 0.932 (2.21) & 0.935 (4.04)  & 1.248 (4.18) & 0.992 (1.94) & 1.147 (2.45)  & 1.643 (2.15) \\
                          & & MQCNN                  & 0.912 (2.07) & 0.916 (3.99)  & 1.222 (4.12) & 0.966 (1.90) & 1.113 (2.41)  & 1.553 (2.16) \\
                          & & MLP                    & 0.945 (2.23) & 1.025 (4.58)  & 1.356 (4.65) & 0.953 (1.87) & 1.069 (2.15)  & 1.521 (1.85) \\
                          & & LSTM                   & 0.920 (2.11) & 0.953 (4.16)  & 1.270 (4.26) & 0.948 (1.87) & 1.065 (2.18)  & 1.510 (1.90) \\
                          & & Transformer            & 1.001 (2.23) & 1.110 (4.47)  & 1.460 (4.54) & 0.952 (1.88) & 1.072 (2.20)  & 1.526 (1.91) \\
                          & & TS2Vec                 & 1.106 (1.86) & 1.101 (4.61)  & 1.302 (4.70) & 1.088 (1.60) & 1.091 (1.84)  & \bf 1.392 (1.63)   \\
\cmidrule{2-9}
& \multirow{3}{*}{\makecell[l]{Ensemble}} & Ensemble (Best)   & 0.908 (2.07) & 0.929 (4.14)  & 1.246 (4.25) & 0.969 (1.72) & 1.021 (1.91)  & 1.399 (1.66) \\
                          & & Deep Ensembles   & 0.930 (2.09) & 0.957 (4.19)  & 1.279 (4.30) & 1.101 (1.76) & 1.152 (2.24)  & 1.580 (1.96) \\
                          & & N-BEATS & 0.889 (2.03) & 0.879 (3.89)  & 1.197 (4.03) &  0.945 (1.90) & 1.062 (2.24)  & 1.525 (1.96) \\
\cmidrule{2-9}  \morecmidrules
\cmidrule{2-9} \ldelim\{{10}{*}[\color{black} {\rotatebox[origin=c]{90}{ zero-shot inference}}\hspace{.45em}]\hspace{.3em} & \multirow{6}{*}{Global} & DeepAR                 & 0.931 (2.23) & 0.943 (4.13)  & 1.267 (4.25) & 0.990 (1.95) & 1.139 (2.37)  & 1.636 (2.06) \\
                          & & MQCNN                    & 0.913 (2.08) & 0.914 (4.03)  & 1.214 (4.17) & 0.957 (1.86) & 1.077 (2.23)  & 1.511 (1.96) \\
                          & & MLP                    & 0.910 (2.03) & 0.943 (4.14)  & 1.260 (4.24) & 0.954 (1.90) & 1.069 (2.21)  & 1.537 (1.91) \\
                          & & LSTM                   & 0.921 (2.02) & 0.950 (4.21)  & 1.245 (4.32) & 0.946 (1.92) & 1.063 (2.22)  & 1.537 (1.93) \\
                          & & Transformer            & 1.021 (2.14) & 1.117 (4.45)  & 1.422 (4.53) & 0.958 (1.93) & 1.079 (2.20)  & 1.559 (1.89) \\
                          & & TS2Vec                 & 1.116 (1.89) & 1.110 (4.48)  & 1.321 (4.57) & 1.082 (1.60) & 1.090 (1.86)  & 1.394 (1.65) \\
\cmidrule{2-9}
& \multirow{3}{*}{\makecell[l]{Ensemble}} & Ensemble (Best)   & 0.900 (2.02) & 0.904 (3.97)  & 1.210 (4.11) & 0.906 (1.86) & 0.983 (1.96)  & 1.444 (1.66) \\
                          & & Deep Ensembles   & 0.946 (1.95) & 0.928 (4.02)  & 1.208 (4.16) & 0.945 (1.89) & 1.061 (2.20)  & 1.511 (1.92) \\
                          & & N-BEATS & 0.892 (2.02) & 0.886 (3.89)  & 1.197 (4.04) & 0.946 (1.90) & 1.063 (2.23)  & 1.521 (1.94) \\
\cmidrule{2-9}
\cmidrule{2-9}
& \bf Ours                      & \bf Forchestra    & \bf 0.882 (1.96) & \bf 0.875 (3.85)  & \bf 1.183 (4.00) & \bf 0.893 (1.84) & \bf 0.965 (1.89)  & 1.408 (1.59) \\
\cmidrule[1.0pt]{2-9}
\end{tabular}
}
\end{table*}

==> tables/tab_transfer_stale.tex <==
\begin{table*}[ht]
\centering
\caption{Forecast accuracy on unseen products. Pre-trained models and Forchestra are trained on the original dataset.}
\label{tab:comp_test}
{\small
\begin{tabular}{ll|ccc|ccc}
\toprule
\multirow{2}{*}{}         & \multirow{2}{*}{Model} & \multicolumn{3}{c|}{\texttt{E-Commerce} (Unseen Items)} & \multicolumn{3}{c}{\texttt{M5} (Unseen Products)}  \\
                          &                        & MASE & MAE & RMSE         & MASE & MAE & RMSE       \\
\midrule
\multirow{3}{*}{Univariate} & ARIMA                  & 1.045 (1.84) & 0.987 (3.83)  & 1.202 (4.01) & 1.108 (1.67) & 1.163 (2.36)  & 1.482 (2.17) \\
                          & Prophet                & 1.112 (1.97) & 1.126 (4.21)  & 1.356 (4.34) & 1.125 (1.66) & 1.172 (2.08)  & 1.501 (1.86) \\
                          & SMA         & 1.145 (2.15) & 1.179 (4.60)  & 1.396 (4.69) & 1.180 (1.92) & 1.413 (2.75)  & 1.843 (2.48) \\
\midrule
\multirow{6}{*}{Multivariate} & DeepAR             & 0.932 (2.21) & 0.935 (4.04)  & 1.248 (4.18) & 0.992 (1.94) & 1.147 (2.45)  & 1.643 (2.15) \\
                          & MQCNN                  & 0.912 (2.07) & 0.916 (3.99)  & 1.222 (4.12) & 0.966 (1.90) & 1.113 (2.41)  & 1.553 (2.16) \\
                          & MLP                    & 0.945 (2.23) & 1.025 (4.58)  & 1.356 (4.65) & 0.953 (1.87) & 1.069 (2.15)  & 1.521 (1.85) \\
                          & LSTM                   & 0.920 (2.11) & 0.953 (4.16)  & 1.270 (4.26) & 0.948 (1.87) & 1.065 (2.18)  & 1.510 (1.90) \\
                          & Transformer            & 1.001 (2.23) & 1.110 (4.47)  & 1.460 (4.54) & 0.952 (1.88) & 1.072 (2.20)  & 1.526 (1.91) \\
                          & TS2Vec                 & 1.106 (1.86) & 1.101 (4.61)  & 1.302 (4.70) & 1.088 (1.60) & 1.091 (1.84)  & \bf 1.392 (1.63)   \\
\midrule
\multirow{2}{*}{\makecell[l]{Ensemble \\ of Supervised}} & Ensemble (Best)   & 0.908 (2.07) & 0.929 (4.14)  & 1.246 (4.25) & 0.969 (1.72) & 1.021 (1.91)  & 1.399 (1.66) \\
                          & Deep Ensembles   & - & -  & - & 1.101 (1.76) & 1.152 (2.24)  & 1.580 (1.96) \\
\midrule  
\midrule
\multirow{6}{*}{Pre-trained} & DeepAR                 & 0.931 (2.23) & 0.943 (4.13)  & 1.267 (4.25) & 0.990 (1.95) & 1.139 (2.37)  & 1.636 (2.06) \\
                          & MQCNN                    & 0.913 (2.08) & 0.914 (4.03)  & 1.214 (4.17) & 0.957 (1.86) & 1.077 (2.23)  & 1.511 (1.96) \\
                          & MLP                    & 0.910 (2.03) & 0.943 (4.14)  & 1.260 (4.24) & 0.954 (1.90) & 1.069 (2.21)  & 1.537 (1.91) \\
                          & LSTM                   & 0.921 (2.02) & 0.950 (4.21)  & 1.245 (4.32) & 0.946 (1.92) & 1.063 (2.22)  & 1.537 (1.93) \\
                          & Transformer            & 1.021 (2.14) & 1.117 (4.45)  & 1.422 (4.53) & 0.958 (1.93) & 1.079 (2.20)  & 1.559 (1.89) \\
                          & TS2Vec                 & 1.116 (1.89) & 1.110 (4.48)  & 1.321 (4.57) & 1.082 (1.60) & 1.090 (1.86)  & 1.394 (1.65) \\
\midrule
\multirow{2}{*}{\makecell[l]{Ensemble \\ of Pre-trained}} & Ensemble (Best)   & 0.900 (2.02) & 0.904 (3.97)  & 1.210 (4.11) & 0.906 (1.86) & 0.983 (1.96)  & 1.444 (1.66) \\
                          & Deep Ensembles   & 0.946 (1.95) & 0.928 (4.02)  & 1.208 (4.16) & 0.945 (1.89) & 1.061 (2.20)  & 1.511 (1.92) \\
\midrule
\midrule
\bf Ours                      & \bf Forchestra    & \bf 0.882 (1.96) & \bf 0.875 (3.85)  & \bf 1.183 (4.00) & \bf 0.893 (1.84) & \bf 0.965 (1.89)  & 1.408 (1.59) \\
\bottomrule
\end{tabular}
}
\end{table*}

==> tables/tab_wmt21_short.tex <==

\begin{table*}[ht]
\centering

\caption{Comparison of translation quality between competition winners by language and our system. The highest scores are highlighted in bold.}
\label{tab:wmt21_short}
{\normalsize
\resizebox{\linewidth}{!}{%
\begin{tabular}{ll|ccccc|c}
\toprule
\multirow{3}{*}{}         & \multirow{3}{*}{System} & \multicolumn{5}{c|}{Terminology-focused} & \multicolumn{1}{c}{Translation Quality}  \\
                          &                        & Exact-Match & Lemmatized-Match & \multicolumn{2}{c}{Window Overlap} & 1-TERm       &        \\
                          &                        & Accuracy (EMA) & Accuracy (LMA) & (2) & (3) &   Score     & BLEU       \\\midrule
\multirow{5}{*}{EN-FR} & PROMT.soft                    & 0.959 & 0.972 & 0.226 & 0.218 & 0.448 &  41.22 \\
                            & M2M100 small baseline & 0.813 & 0.838 &  0.191 & 0.188 & 0.409 & 35.38 \\
                            & M2M100 small cascaded          & 0.985 & 0.990 &  0.207 & 0.207 & 0.408 & 35.21\\
                            & M2M100 small GBS & 0.989 & 0.993 & 0.158 & 0.160 & 0.207 & 21.86 \\
                            & M2M100 large baseline & 0.880 & 0.899 & 0.231 & 0.225 & 0.442 & 40.15 \\
                            & M2M100 large cascaded          & \textbf{0.991} & \textbf{0.994} & 0.240 & 0.236 & 0.444 & 40.51\\
                            & M2M100 large GBS & 0.994 & 0.996 & 0.185 & 0.183 & 0.309 & 27.76 \\\cmidrule{2-8}
                            & NLLB & 0.903 & 0.922 & \textbf{0.340} & \textbf{0.334} & \textbf{0.568} & \textbf{46.68}\\

\midrule
\multirow{5}{*}{EN-RU} & PROMT.soft                    & 0.862 & 0.913 & 0.176 & 0.174 & 0.315 & \textbf{31.22} \\
                            & M2M100 small baseline & 0.682 & 0.725 & 0.136 & 0.132 & 0.274 & 23.89 \\
                            & M2M100 small cascaded          & 0.916 & 0.934 & 0.150 & 0.151 & 0.273 & 23.73\\
                            & M2M100 small GBS & 0.963 & 0.969 & 0.121 & 0.120 & 0.0 & 12.01 \\
                            & M2M100 large baseline & 0.753 & 0.797 & 0.154 & 0.152 & 0.300 & 29.09 \\
                            & M2M100 large cascaded          & \textbf{0.925} & \textbf{0.950} & 0.176 & 0.177 & 0.404 & 29.22\\
                            & M2M100 large GBS & 0.973 & 0.982 & 0.136 & 0.137 & 0.127 & 16.56 \\\cmidrule{2-8}
                            & NLLB & 0.782 & 0.827 & \textbf{0.217} & 0.211 & \textbf{0.419} & 27.76\\

\bottomrule
\end{tabular}
}
}
\end{table*}
